Neural Directional Encoding for Efficient and Accurate View-Dependent Appearance Modeling

Novel-view synthesis of specular objects like shiny metals or glossy paints remains a significant challenge. Not only the glossy appearance but also global illumination effects, including reflections of other objects in the environment, are critical components to faithfully reproduce a scene. In this paper, we present Neural Directional Encoding (NDE), a view-dependent appearance encoding of neural radiance fields (NeRF) for rendering specular objects. NDE transfers the concept of feature-grid-based spatial encoding to the angular domain, significantly improving the ability to model high-frequency angular signals. In contrast to previous methods that use encoding functions with only angular input, we additionally cone-trace spatial features to obtain a spatially varying directional encoding, which addresses the challenging interreflection effects. Extensive experiments on both synthetic and real datasets show that a NeRF model with NDE (1) outperforms the state of the art on view synthesis of specular objects, and (2) works with small networks to allow fast (real-time) inference. The project webpage and source code are available at: \url{https://lwwu2.github.io/nde/}.

==> equations/cone_tracing.tex <==
\begin{equation}
    \sigma_g^i,\mathbf{h}_g^i=
\text{MLP}(\mathbf{h}_g(\mathbf{x}'_i,\lambda_i)),\lambda_i=\log_2(r_i).
\label{eq:cone-tracing}
\end{equation}

==> equations/spatio-spatial.tex <==
\begin{equation}
    \mathbf{c}_s(\mathbf{x},\bm{\omega}_r)=\mathbf{c}_s(\mathbf{x},\mathbf{x}')
    =\text{MLP}(\mathbf{f}(\mathbf{x}),\mathbf{f}(\mathbf{x}')).
\end{equation}

==> rebuttal/flip.tex <==
\begin{table}[t]
    \centering
    \caption{
        FLIP metric on synthetic scenes.
    }
    \label{tab:rebuttal-flip}
    \setlength\tabcolsep{2 pt}
    \resizebox{0.99\linewidth}{!}{
        \begin{tabular}{l c c c c c c c c}
        \toprule
        \textbf{Method} & \textbf{Mat.} & \textbf{Teapot} & \textbf{Toaster} & \textbf{Car} & \textbf{Ball} & \textbf{Coffee} & \textbf{Helmet} & \textbf{Mean} \\
        \midrule
        NeRO & 0.082 & 0.012 & \snd{0.097} & \snd{0.049} & 0.058 & 0.039 & 0.083 & 0.060 \\
        ENVIDR & 0.062 & 0.030 & 0.098 & 0.056 & \snd{0.037} & 0.046 & \snd{0.049} & 0.054 \\
        Ref-NeRF & \fst{0.023} & \snd{0.011} & 0.108 & 0.071 & 0.038 & \fst{0.030} & 0.072 & \snd{0.050} \\
        3DGS & 0.042 & \fst{0.007} & 0.153 & 0.051 & 0.104 & \snd{0.032} & 0.073 & 0.066\\
        
        \textbf{NDE (ours)} & \snd{0.039} & \fst{0.007} & \fst{0.065} & \fst{0.038} & \fst{0.027} & 0.035 & \fst{0.035} & \fst{0.035}\\
        \bottomrule
        \end{tabular}
    }
\end{table}

==> rebuttal/hashgrid.tex <==
\begin{table}[t]
    \centering
    \caption{
        Comparison of geometry encoding on synthetic scenes in PSNR. ``Pos. enc.'' denotes positional encoding.
    }
    \label{tab:rebuttal-hashgrid}
    \setlength\tabcolsep{2 pt}
    \resizebox{1\linewidth}{!}{
        \begin{tabular}{l c c c c c c c c}
        \toprule
        \textbf{Method} & \textbf{Mat.} & \textbf{Teapot} & \textbf{Toaster} & \textbf{Car} & \textbf{Ball} & \textbf{Coffee} & \textbf{Helmet} & \textbf{Mean} \\
        \midrule
        Hashgrid & 30.12 & 46.46 & 25.83 & 29.94 & 36.41 & 33.25 & 34.08 & 33.73\\
        Pos. enc. & \fst{31.53} & \fst{49.12} & \fst{30.32} & \fst{30.39} & \fst{44.66} & \fst{36.57} & \fst{37.77} & \fst{37.19}\\
        \bottomrule
        \end{tabular}
    }
\end{table}

==> rebuttal/ref_real_tab.tex <==
\begin{table}[t]
    \centering
    \caption{
        PSNR on the Ref-NeRF garden spheres scene.
    }
    \label{tab:ref-real}
    \setlength\tabcolsep{4 pt}
    \resizebox{0.7\linewidth}{!}{
        \begin{tabular}{l c c c}
        \toprule
        &ENVIDR & Ref-NeRF & \textbf{NDE (ours)}\\
        \midrule
        \textbf{PSNR}$\uparrow$&
        22.67 & \snd{23.46} & \fst{23.63}\\
        \bottomrule
        \end{tabular}
    }
    \vspace{3mm}
\end{table}

==> rebuttal/reflection_field.tex <==
\begin{figure}[t]
    \centering
    \setlength\tabcolsep{0.5pt}
    \resizebox{1.0\linewidth}{!}{
        \begin{tabular}{cc}
            \includegraphics[width=0.35\linewidth]{rebuttal/reflection_query.pdf}&
            \includegraphics[width=0.7\linewidth]{rebuttal/reflection_field.pdf}\\
        \end{tabular}
    }
    \caption{
        Visualization of near- and far-field reflection over hemisphere (right) at the queried location (left).
    }
    \label{fig:ref-field}
    \vspace{3mm}
\end{figure}
